Learn 2 Rage: Experiencing The Emotional Roller Coaster That Is Reinforcement Learning

This work presents the experiments and solution outline for our teams winning submission in the Learn To Race Autonomous Racing Virtual Challenge 2022 hosted by AIcrowd. The objective of the Learn-to-Race competition is to push the boundary of autonomous technology, with a focus on achieving the safety benefits of autonomous driving. In the description the competition is framed as a reinforcement learning (RL) challenge. We focused our initial efforts on implementation of Soft Actor Critic (SAC) variants. Our goal was to learn non-trivial control of the race car exclusively from visual and geometric features, directly mapping pixels to control actions. We made suitable modifications to the default reward policy aiming to promote smooth steering and acceleration control. The framework for the competition provided real time simulation, meaning a single episode (learning experience) is measured in minutes. Instead of pursuing parallelisation of episodes we opted to explore a more traditional approach in which the visual perception was processed (via learned operators) and fed into rule-based controllers. Such a system, while not as academically "attractive" as a pixels-to-actions approach, results in a system that requires less training, is more explainable, generalises better and is easily tuned and ultimately out-performed all other agents in the competition by a large margin.

==> Abstract.tex <==
\subsection{Abstract}
\label{sec:abstract}
This work presents the experiments and solution outline for the winning submission in the Learn To Race Autonomous Racing Virtual Challenge 2022. The objective of the Learn-to-Race competition is to push the boundary of autonomous technology, with a focus on achieving the safety benefits of autonomous driving. In the description the competition is framed as a reinforcement learning (RL) challenge. 

We focused out initial efforts on implementation of Soft Actor Critic (SAC) variants. Our goal was to learn non-trivial control of the race car exclusively from visual and geometric features, directly mapping pixels to control actions. We made suitable modifications to the default reward policy aiming to promote smooth steering and acceleration control.

The framework for the competition provided real time simulation, meaning a single episode (learning experience) is measured in minutes. Instead of pursuing parallelisation of episodes we opted to explore a more traditional approach in which the visual percepts were processed (via learned operators) and fed into a rule-base controllers. 

Such a system, while not as academically ``pure'' as a pixels-to-actions approach, results in a system that requires less training, is more explainable, generalises better, is more easily tuned and ultimately out-performed all other agents in the competition by a large margin.

==> Tables.tex <==
\begin{table}
    \centering
    \begin{tabular}{l c c| c c}
        \hline
        Track  & $fps$ & local kph & $fps$ & eval kph \\
        \hline
        Vegas North Road   &     &        & 5.1 & 92.54 \\
        Anglesey National & 7.0 & 103.97 &     &       \\
        Thruxton         & 7.0 & 147.12 &     &       \\
        \hline
    \end{tabular}
    \caption{Track times with location classifier, $fps$ frames per second, local or evaluation (AIcrowd) refers to simulator location}
    \label{tab:track_times_post}
\end{table}

==> layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}
